Detecting Multimodal Situations with Insufficient Context and Abstaining from Baseless Predictions

Despite the widespread adoption of Vision-Language Understanding (VLU) benchmarks such as VQA v2, OKVQA, A-OKVQA, GQA, VCR, SWAG, and VisualCOMET, our analysis reveals a pervasive issue affecting their integrity: these benchmarks contain samples where answers rely on assumptions unsupported by the provided context. Training models on such data foster biased learning and hallucinations as models tend to make similar unwarranted assumptions. To address this issue, we collect contextual data for each sample whenever available and train a context selection module to facilitate evidence-based model predictions. Strong improvements across multiple benchmarks demonstrate the effectiveness of our approach. Further, we develop a general-purpose Context-AwaRe Abstention (CARA) detector to identify samples lacking sufficient context and enhance model accuracy by abstaining from responding if the required context is absent. CARA exhibits generalization to new benchmarks it wasn't trained on, underscoring its utility for future VLU benchmarks in detecting or cleaning samples with inadequate context. Finally, we curate a Context Ambiguity and Sufficiency Evaluation (CASE) set to benchmark the performance of insufficient context detectors. Overall, our work represents a significant advancement in ensuring that vision-language models generate trustworthy and evidence-based outputs in complex real-world scenarios.

==> graphs/vlu_benchmark_examples.tex <==
\begin{figure*}[h!]
    % \vspace{-4cm}
    \centering
    \captionsetup{skip=5pt}
    % \scalebox{1}{
    \includegraphics[width=\linewidth]{graphs/pdf_files/vlu_benchmark_examples_v1.pdf}
    % }
    % \vspace{-4cm}
    \caption {
    % Examples with insufficient event-specific context commonly exist across popular VLU benchmarks. Without sufficient context, VLMs tend to make hallucinated predictions. After applying CARA, as the VLMs robot wears the CARA hat, VLMs can abstain from making baseless responses.
    % Samples with insufficient context generally exist across benchmarks and are difficult to avoid.
    Instances lacking sufficient event-specific context are prevalent across widely-used VLU benchmarks. In scenarios with inadequate context, VLMs are prone to producing hallucinated predictions. However, with the implementation of CARA, VLMs are equipped to abstain from making baseless responses, effectively wearing the 'CARA hat' to enhance decision-making accuracy.
    }
    \label{fig:vlu_examples}
\end{figure*}

==> tables/context_adding_methods.tex <==

\begin{table}[h!]\small
    \caption{Comparison between different methods of adding context. Models with Prob selection shows significant improvement.}
    \fontsize{8}{9}\selectfont
    \setlength{\tabcolsep}{0.9pt}
    \captionsetup{skip=5pt}
    \centering
    \begin{tabular}{lll}
        \toprule
        Model                   & Visual SWAG        & VCR \\
        \midrule
        VL-BERT & 74.2 & 70.18 \\
        VL-BERT+Fixed Index     & 77.86     & 72.10  \\
        VL-BERT+Random Index  & 76.79     & 72.20 \\
        VL-BERT+Prob Selection & \textbf{78.40} & \textbf{73.78} \\
        \midrule
        BLIP&62.65&69.03 \\
        BLIP+Fixed Index     &  62.85    & 67.60  \\
        BLIP+Random Index  & 61.23    & 68.03 \\
        BLIP+Prob Selection  &\textbf{63.22}&\textbf{70.74}\\
        \bottomrule
    \end{tabular}
    \label{table:context_adding_method}
\end{table}

==> tables/context_selection_method.tex <==
\begin{table} [h!]\small
    \centering
    \caption{Ablation of context selection methods. The top half selects context using language models. The bottom half tests the effect of contexts based on the index. }
    \fontsize{8}{9}\selectfont
    \setlength{\tabcolsep}{3pt}
    \captionsetup{skip=5pt}
    \begin{tabular}{l|l|l}
        \toprule
        Selection Method & V. SWAG & VCR \\
        \midrule
        Embedding Similarity &76.91 &72.44\\
        Prob Selection & \textbf{78.4} &\textbf{73.78}\\
        \midrule
        Random Selection & 76.79 &71.43\\
        Index -1 & 77.86 & 71.76\\
        Index -2 & 77.25 & 71.01\\
        Index -3 & 76.15 & 70.23\\
        \bottomrule
    \end{tabular}
    \label{table:selection_method}
\end{table}

==> tables/unused/abstain_generalization.tex <==
\begin{figure}
\centering
  %\begin{minipage}[t]{0.48\linewidth}
   % \input{tables/abstain_generalization_v1}
  %\end{minipage}
  %\hfill
  \begin{minipage}[t]{1\linewidth}
    % \vspace{-2.4cm}
    % \includegraphics[width=\textwidth]{images/cur_accVsdatasize3.png}
    \input{tables/abstain_generalization_v2}
  \end{minipage}
\end{figure}

==> tables/unused/llm_selection_number.tex <==
\begin{table*}[h!]\small
    \caption{Selection number of large language models.}
    \centering
    \captionsetup{skip=5pt}
    \begin{tabular}{l|l|l|l|lll}
    \hline
        \multirow{2}{*}{Model}& \multirow{2}{*}{Selection Num}&V.SWAG&VCR&\multicolumn{3}{c}{VisualCOMET} \\
        &&Accuracy&Accuracy&BLEU4&CIDER&METEOR\\
        \hline
        \multirow{4}{*}{BLIP}&3 Select 0&84.58&78.20&0.1225&0.4631&0.1683\\
        \cline{2-7}
        &3 Select 1&86.13&81.10&0.1265&0.4743&0.1699\\
        \cline{2-7}
        &3 Select 2&\textbf{86.62}&\textbf{81.32}&\textbf{0.1296}&\textbf{0.4787}&\textbf{0.1708}\\
        \cline{2-7}
        &3 Select 3&86.52&80.93&0.1284&0.4766&0.1704\\
        \hline
        
        \multirow{4}{*}{MiniGPT-4}&3 Select 0&85.92&81.42&0.1430&0.4694&0.1701\\
        \cline{2-7}
        &3 Select 1&87.16&82.15&0.1440&0.4758&0.1707\\
        \cline{2-7}
        &3 Select 2&\textbf{87.21}&\textbf{83.80}&\textbf{0.1457}&\textbf{0.4822}&\textbf{0.1713}\\
        \cline{2-7}
        &3 Select 3&87.03&83.49&0.1437&0.4793&0.1710\\
        \hline
    \end{tabular}
    \label{table:main_result}
\end{table*}

==> tables/unused/selection_number.tex <==
\begin{figure}[h!]\small
\captionsetup{skip=5pt}
\begin{tikzpicture}
\begin{axis}[
    width=0.48\textwidth,
    height=0.32\textwidth,
    title={Selection Number Experiments},
    xlabel={Selection Number},
    ylabel={Accuracy},
    xmin=0, xmax=6,
    ymin=51, ymax=72,
    xtick={0,1,...,6},
    ytick={52,54,...,72},
    grid=both,legend style={at={(1,-0.3)},anchor=south east, font=\tiny},
]
    \definecolor{swag}{rgb}{0.0, 0.53, 0.74}
    \definecolor{vcr}{rgb}{0.67, 0.31, 0.32}
    \addplot[color=swag,mark=*, mark size=2pt,line width=1.5pt] coordinates {
        (0,52.27)
        (1,61.18)
        (2,59.61)
        (3,58.15)
        (4,54.64)
    };
    \addlegendentry{Visual SWAG}
    
    \addplot[color=vcr,mark=*, mark size=2pt,line width=1.5pt] coordinates {
        (0,69.03)
        (1,69.72)
        (2,70.82)
        (3,70.67)
        (4,69.28)
        (5,68.72)
    };
    \addlegendentry{VCR}
\end{axis}
\end{tikzpicture}
\caption{Ablation study for context selection number. The peak in the accuracy indicates the optimal context selection number.}
\label{fig:selection_number}
\end{figure}
